Cubic graphs with no eigenvalues in the interval (-1,1)

We give a complete characterisation of the cubic graphs with no eigenvalues in the open interval $(-1,1)$. There are two infinite families, one due to Guo and Mohar [Linear Algebra Appl. 449:68--75] the other due to Koll\'ar and Sarnak [Communications of the AMS. 1,1--38], and $14$ "sporadic" graphs on at most $32$ vertices. This allows us to show that $(-1,1)$ is a maximal spectral gap set for cubic graphs. Our techniques including examination of various substructure and an application of the classification of generalized line graphs.

==> girth8.tex <==
In this section we show that all cubic bipartite graphs of girth at least $8$ have an eigenvalue in the interval $(-1,1)$. In each case we accomplish this by identifying a subset $S$ of the vertices such that the principal minor of $A(G)^2 - I$ with rows and columns indexed by $S$ is negative.

Throughout we will use $M(G)$ or just $M$ to denote $A(G)^2-I$ and $M_{SS}$ to denote the submatrix of $M$ with rows and columns indexed by $S$. The diagonal entries of $M_{SS}$ are all equal to $2$ while the $(v,w)$-entry  of $M_{SS}$ is equal to the number of paths of length $2$ from $v$ to $w$. Note that the count of $2$-paths between $v$ and $w$ includes paths whose intermediate vertex is not in $S$.


\subsubsection{Girth equal to 8}

Let $G$ be a cubic bipartite graph of girth 8 and let $C = \{v_0,v_1,\ldots,v_7\}$ be a cycle of length $8$ in $G$. Then let $v_8$ be the neighbour of $v_0$ not in $C$ and $v_9$ be a neighbour of $v_8$, also not in $C$, leading to the configuration in the left-hand image of \cref{eightcycle}. Due to the girth constraint there are no paths of length $2$ in $G$ that use a vertex outside $\{v_0,v_1,\ldots,v_9\}$ with the possible exception of a path from $v_4$ to $v_9$ using an additional vertex $v_{10}$ as depicted in the right-hand image of \cref{eightcycle}. 

\begin{figure}
\begin{center}
\begin{tikzpicture}
\draw [white] (-2.5,-2.5) rectangle (2.5,3.5);
\tikzstyle{vertex}=[fill=blue!25, circle, draw=black, inner sep=0.8mm]
\foreach \x in {0,1,...,7} {
  \node [vertex] (v\x) at (90+45*\x:2cm) {};
}
\node [vertex] (v8) at (0,1) {};
\node [vertex] (v9) at (0,0) {};
\draw (v0)--(v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v0);
\draw (v0)--(v8)--(v9);

% \foreach \x in {0,2,4,6} {
% \filldraw [draw=black,fill=red,opacity=0.5] (v\x) circle (2.2mm) ;
% }

% \filldraw [draw=black,fill=red,opacity=0.5] (vx) circle (2.2mm) ;

\node [above right] at (v0) {$v_0$};
\node [above left] at (v1) {$v_1$};
\node [above left] at (v2) {$v_2$};
\node [below left] at (v3) {$v_3$};
\node [below left] at (v4) {$v_4$};
\node [below right] at (v5) {$v_5$};
\node [above right] at (v6) {$v_6$};
\node [above right] at (v7) {$v_7$};
\node [above right] at (v8) {$v_8$};
\node [above right] at (v9) {$v_9$};

\fill [yellow] (v0) circle (1mm) ;
\fill [yellow] (v2) circle (1mm) ;
\fill [yellow] (v4) circle (1mm) ;
\fill [yellow] (v6) circle (1mm) ;
\fill [yellow] (v9) circle (1mm) ;


\end{tikzpicture}
\hspace{1cm}
\begin{tikzpicture}
\draw [white] (-2.5,-2.5) rectangle (2.5,3.5);
\tikzstyle{vertex}=[fill=blue!25, circle, draw=black, inner sep=0.8mm]
\foreach \x in {0,1,...,7} {
  \node [vertex] (v\x) at (90+45*\x:2cm) {};
}
\node [vertex] (v8) at (0,1) {};
\node [vertex] (v9) at (0,0) {};
\node [vertex] (v10) at (0,-1) {};

\draw (v0)--(v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v0);
\draw (v0)--(v8)--(v9);
\draw (v4)--(v10)--(v9);


% \foreach \x in {0,2,4,6} {
% \filldraw [draw=black,fill=red,opacity=0.5] (v\x) circle (2.2mm) ;
% }


% \filldraw [draw=black,fill=red,opacity=0.5] (vx) circle (2.2mm) ;

\node [above right] at (v0) {$v_0$};
\node [above left] at (v1) {$v_1$};
\node [above left] at (v2) {$v_2$};
\node [below left] at (v3) {$v_3$};
\node [below left] at (v4) {$v_4$};
\node [below right] at (v5) {$v_5$};
\node [above right] at (v6) {$v_6$};
\node [above right] at (v7) {$v_7$};
\node [above right] at (v8) {$v_8$};
\node [above right] at (v9) {$v_9$};

\node [above right] at (v10) {$v_{10}$};

\fill [yellow] (v0) circle (1mm) ;
\fill [yellow] (v2) circle (1mm) ;
\fill [yellow] (v4) circle (1mm) ;
\fill [yellow] (v6) circle (1mm) ;
\fill [yellow] (v9) circle (1mm) ;


\end{tikzpicture}
\end{center}
\caption{Configurations in a cubic graph of girth 8}
\label{eightcycle}
\end{figure}

Now if $S = \{v_0, v_2, v_4, v_6, v_9\}$ then the submatrix of $A(G)^2-I$ indexed by $S$ is either $M_1$ or $M_2$ where
\[
M_1 = \left[
\begin{array}{ccccc}
2&1&0&1&1\\
1&2&1&0&0\\
0&1&2&1&0\\
1&0&1&2&0\\
1&0&0&0&2
\end{array}
\right],
\qquad
M_2 = \left[
\begin{array}{ccccc}
2&1&0&1&1\\
1&2&1&0&0\\
0&1&2&1&{\color{red}1}\\
1&0&1&2&0\\
1&0&{\color{red}1}&0&2
\end{array}
\right].
\]

As $\det M_1 = -4$ and $\det M_2 = -16$ the matrix $A^2-I$ is not positive semi-definite.



==> intro.tex <==
\section{Introduction}


%%%% introduction paragraph: motivation comes from chemical graph theory and also the related study of ALon-Boppana type spectral gaps 

We show that, with the exception of  two infinite families and 14 sporadic examples, all connected cubic graphs have an eigenvalue in the open interval $(-1,1)$.
\krystalsays{We will begin by motivating our study in the context of chemical graph theory and spectral gap story. }
%%% chemical graph theory, HOMO-LUMO

A \textsl{chemical graph} is a connected, simple, subcubic graph. 
motivation from H\"{u}ckel theory \krystalsays{(? model?) }
Fowler and Pisanski \cite{FowPis2010} studied the  HOMO-LUMO separation, which is the gap between the  highest occupied molecular orbital (HOMO) and lowest unoccupied molecular orbital (LUMO). Let $G$ be a graph on $n$ vertices and let 
\[ \lambda_1 \geqslant \lambda_2 \geqslant \cdots \geqslant \lambda_n
\]
be the eigenvalues of the adjacency matrix of $A$ in non-increasing order. The eigenvalues in the HOMO-LUMO separation, also known as the \textsl{median eigenvalues}, are $\lambda_H, \lambda_L$ where 
\[\lambda_{H} = \lambda_{L} = \lambda_{\nicefrac{n+1}{2}} \]
when $n$ is odd and 
\[\lambda_{H} = \lambda_{\nicefrac{n}{2}}, \quad \lambda_{L}= \lambda_{\nicefrac{n}{2} + 1} \]
when $n$ is even. The HOMO-LUMO separation studied in \cite{FowPis2010} and following works,  is the gap  $|\lambda_{H} - \lambda_{L} |$ and graphs with larger gaps are considered to have greater stability. 
The \textsl{HL-index} of a graph, denoted $R(G)$, is defined as follows:
\[
R(G) = \max \{ |\lambda_H|, |\lambda_L| \}. 
\]
For each graph, we can consider the pair $(\lambda_H, \lambda_L)$. Fowler and Pisanski consider the \textsl{chemical triangle} to be the triangle in the $xy$-plane with vertices $(-1,-1)$,  $(1,-1)$ and  $(1,1)$. The main question concerned graphs for which  $(\lambda_H, \lambda_L)$ lies in the chemical triangle and they state that it is ``a plausible conjecture'' that  all but a finite number of exceptions lie within the chemical triangle, or, equivalently, that $R(G) \leq 1$ for all but a finite number of subcubic graphs.  We will return to the chemical triangle, with the results of this paper, in Figure \ref{fig:chemicaltriangle}. \krystalsays{It remain open to show subcubic graphs, apart from finite exception, have $R(G)\leq 1$. Partial results, our result gives an alternate for cubic bipartite case, etc. Our results show that all cubic graphs, except Heawood, do have an eigenvalue in $[-1,1]$, but we do not know that the median one is there. }

% bipartite results only 
%bipartite graphs, odd vertices have 0, even number of vertices, symmetric. 
Since the adjacency eigenvalues of bipartite graphs are symmetric about $0$, studying $R(G)$ reduces to finding symmetric intervals $(-\alpha,\alpha)$ which do not contain any eigenvalue -- and thus the median eigenvalue --  of graphs in certain bipartite graph classes. 
%lower bounding $R(G)$ is equivalent to finding symmetric intervals $(-\alpha,\alpha)$ which do not contain any eigenvalu
In \cite{Moh2013}, Mohar shows that the median eigenvalues  of all bipartite subcubic planar graphs lie in $[-1,1]$.
In \cite{Moh2016}, he shows the same statement for bipartite subcubic graphs, except the Heawood graph. 
In \cite{GuoMoh2014}, an infinite family of cubic bipartite graphs which have no eigenvalues in the open interval $(-1,1)$ is constructed.

% subcubic planar story with outerplanar, K4-free results 
Lower and upper bounds on the maximum value of the HL-index among all graphs with given average degree is given in \cite{Moh2015}. In the same paper, it is shown that a positive fraction of the eigenvalues of a subcubic graph lies in the interval $[-\sqrt{2}, \sqrt{2}]$. 
It is an open problem in \cite{Moh2013} to show that the median eigenvalues of subcubic planar graphs lie in $[-1,1]$. It is true for subcubic, planar, $K_4$-free, see \cite{WanZha2024}. 


%% spectral gaps, Kollar-Sarnak, etc. 
The problem of considering classes of graphs  $\cG$ and real intervals which contain no eigenvalue of any $G \in \cG$ also arises as a spectral gap problem, which arises from the theory surrounding the well-known Alon-Boppana Theorem. 
An open subset $I$ of the reals is a \textsl{(spectral) gap set}  if there infinitely many graphs which have no eigenvalues in $I$. This definition appear in \cite{KolSar2021}, which then focuses on finding maximal gap sets.

The Alon-Boppana theorem states that that for every $\epsilon >0$ and every integer $d \geq 3$, there are only finitely many $d$-regular graphs  where the second largest eigenvalues $\lambda_2$ of the adjacency matrix satisfies $\lambda_2 < 2\sqrt{d-1} -\epsilon$. See \cite{Alo1986, HooLinWig2006,Cio2006,Moh2010}. This theorem  has many implications and is a reason why  the quantity $2\sqrt{d-1}$ also appears in the definition of Ramanujan graphs, which are $d$-regular graphs with $\lambda_2 \leq  2\sqrt{d-1}$, which were first shown to exist in \cite{DavSarVal2003}. 
In terms of spectral gaps, the existence of cubic Ramanujan graphs \cite{Chi1992}, together with the  bound given in \cite{Nil1991} implies that the interval $(2\sqrt{2},3)$, is maximal gap set. The interval $(-1,1)$ is shown to be a maximal spectral gap in \cite{KolSar2021}; the results about median eigenvalues of cubic mentioned above, \cite{Moh2016, GuoMoh2014} established that $(-1,1)$ is a maximal spectral gap when restricted to bipartite cubic  graphs. 

%Additional works in this vein: \cite{AbdGho2023} 

%%%%%%%%%%% our contributions are ...

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\linewidth]{chemical-triangle.pdf}
    \caption{The chemical triangle and some graphs where $(\lambda_H,\lambda_L)$ lies on or outside the boundary.}
    \label{fig:chemicaltriangle}
\end{figure}


%%%%%%%%%%%% organization of the paper 
